Runtime Optimization of Join Location in Parallel Data Management Systems

Applications running on parallel systems often need to join a streaming relation or a stored relation with data indexed in a parallel data storage system. Some applications also compute UDFs on the joined tuples. The join can be done at the data storage nodes, corresponding to reduce side joins, or by fetching data from the storage system to compute nodes, corresponding to map side join. Both may be suboptimal: reduce side joins may cause skew, while map side joins may lead to a lot of data being transferred and replicated. In this paper, we present techniques to make runtime decisions between the two options on a per key basis, in order to improve the throughput of the join, accounting for UDF computation if any. Our techniques are based on an extended ski-rental algorithm and provide worst-case performance guarantees with respect to the optimal point in the space considered by us. Our techniques use load balancing taking into account the CPU, network and I/O costs as well as the load on compute and storage nodes. We have implemented our techniques on Hadoop, Spark and the Muppet stream processing engine. Our experiments show that our optimization techniques provide a significant improvement in throughput over existing techniques.

==> background.tex <==
\section{Background}
Over the past decade, MapReduce has emerged as a popular paradigm for batch 
processing of large volumes of data on a cluster of machines.
While Apache Hadoop has become the most popular implementation of MapReduce, 
other frameworks like SCOPE~\cite{scope}, 
Hyracks~\cite{hyracks} and Spark~\cite{spark} have also emerged.
These systems are designed to work with humongous amounts of data stored in a 
distributed file system. 
Data from distributed files flows through the functions defined by user 
applications in the specific framework.




Some applications using the MapReduce paradigm, like MapReduce joins and entity 
annotations on a 
large corpus of data, may need to join data from multiple sources and evaluate some 
function based 
on data from both sources. For this purpose data from all sources needs to be pipelined 
through a 
set of distributed operators. 



An alternate way is to use the MapReduce framework for only one data 
source,  and store data from the other data sources in some remote datastore. 
For the data stored in the remote datastore, only necessary data needed to join with the 
values in the first source can be fetched from datastore. 


Another paradigm of computing that has become quite popular in the past few years is 
stream data 
processing for large volumes of fast data in a massively parallel manner.
These include Storm~\cite{storm} and Heron~\cite{heron} by Twitter, S4~\cite{s4} by 
Yahoo!, 
Muppet~\cite{muppet} by WalmartLabs, Kinesis~\cite{kinesis} by Amazon, Samza~\cite{samza} 
by 
Linkedin and MillWheel~\cite{millwheel} by Google. 
The focus of these systems is to process the incoming tuples with low latency.
They process recent data and compute aggregates based on these values to find recent 
trends and 
predict trends in the near future. 

For a number of streaming applications need to access historical data that is stored in a 
database and compute functions based on it. Accessing historical data for streaming data 
falls can be thought of as join between streams and relations.
%Applications based on these platforms would be able to see beyond recent history if they 
%are able to access stored data.
%Such applications could potentially perform more complex operations than doing simple 
%aggregation 
%and trend computations. 
However accessing stored data imposes a high cost because of disk I/Os and network calls 
(if the datastore is remote) and hence must be done efficiently. The Stanford STREAM 
system \cite{stream:report}
supports, which is a single node stream processing system, supports joins between streams 
and relations.
However, to the best our knowledge, little research has been done to optimize joins 
between streams and relations.
%The Stanford STREAM system query language, CQL \cite{cql} provides
%support for joining streaming relations with stored relations. 

